Asymptotics of MAP Inference in Deep Networks

Deep generative priors are a powerful tool for reconstruction problems with complex data such as images and text. Inverse problems using such models require solving an inference problem of estimating the input and hidden units of the multi-layer network from its output. Maximum a priori (MAP) estimation is a widely-used inference method as it is straightforward to implement, and has been successful in practice. However, rigorous analysis of MAP inference in multi-layer networks is difficult. This work considers a recently-developed method, multi-layer vector approximate message passing (ML-VAMP), to study MAP inference in deep networks. It is shown that the mean squared error of the ML-VAMP estimate can be exactly and rigorously characterized in a certain high-dimensional random limit. The proposed method thus provides a tractable method for MAP inference with exact performance guarantees.

==> MLVAMP MAP/abstract.tex <==
\begin{abstract}
Deep generative priors are a powerful tool for reconstruction problems
with complex data such as images and text.  Inverse problems using such models
require solving an inference problem of estimating the input and hidden units of the
multi-layer network from its output.  Maximum a priori (MAP) estimation is a
widely-used inference method as it is straightforward to implement, and
has been successful in practice.  However, rigorous
analysis of MAP inference in multi-layer networks is difficult.
This work considers a recently-developed method, multi-layer
vector approximate message passing (ML-VAMP), to study MAP inference in deep networks.
It is shown that the mean squared error of the
ML-VAMP estimate can be exactly and rigorously characterized
in a certain high-dimensional random limit.  The proposed method thus
provides a tractable method for MAP inference with exact performance guarantees.
\end{abstract}

==> MLVAMP MAP/appendices.tex <==
%\begin{appendices}


\section{Proof of Theorem~\ref{thm:mapfix}} \label{sec:mapfixpf}

The linear equalities in \eqref{eq:defines} can be rewritten as,
\begin{subequations}  \label{eq:defr}
\begin{align}
    \rbf_{k\ell}^+ &= \zbfhat^+_{k\ell} + \frac{1}{\alpha^{-}_{k\ell}}\sbf^{+}_{k\ell}
          \\
    \rbf_{k+1,\ell}^- &= \zbfhat^-_{k\ell} - \frac{1}{\alpha^{+}_{k\ell}}\sbf^{-}_{\kp1,\ell} %    \label{eq:definern}
\end{align}
\end{subequations}
Substituting \eqref{eq:defr}  in lines \ref{line:rp} and \ref{line:rn} of Algorithm \ref{algo:ml-vamp} give the updates \eqref{eq:admmsp} and \eqref{eq:admmsn} in Theorem \ref{thm:mapfix}. It remains to show that the optimization problem in updates
\eqref{eq:admmHp} and \eqref{eq:admmHn} is equivalent to
\eqref{eq:mapEnergy_l}. It suffices to show that the terms dependent on $(z_{\ell-1}^-,z^{+}_\ell)$ in both the objective functions $J_\ell$ from \eqref{eq:mapEnergy_l} and $\mc L_\ell$ from \eqref{eq:admmHp} and \eqref{eq:admmHn} are identical. This follows immediately on substituting \eqref{eq:defr} in \eqref{eq:defineEnergy_l}.

It now suffices to show that any fixed point of Algorithm~\ref{algo:ml-vamp} is a critical point of the augmented Lagrangian in \eqref{eq:Lagdef}.
Since we are looking only at fixed points, we can drop the dependence
on the iteration $k$.  So, for example, we can write $\rbf_\ell^+$ for $\rbf_{k\ell}^+$.
To show that $\zbfhat^+_\ell,\zbfhat^-_\ell$ are critical points of the
constrained optimization~\eqref{eq:Fmincon}, we need to show that
there exists dual parameters $\sbf_\ell$ such that for all $\ell=0,\ldots,\Lm1$,
\beq \label{eq:zcon}
    \zbfhat^+_\ell=\zbfhat^-_\ell,
\eeq
\beq \label{eq:Laggrad}
    \frac{\partial \mc L(\zbfhat^+,\zbfhat^-,\sbf)}{\partial \zbf^+_\ell}=0, \quad
    \frac{\partial \mathcal{L} (\zbfhat^+,\zbfhat^-,\sbf)}{\partial \zbf^-_\ell}=0,
\eeq
where $\mc L(\cdot)$ is the Lagrangian in \eqref{eq:Lagdef}.

We first prove \eqref{eq:zcon} whereby primal feasibility is satisfied.
At any fixed point of \eqref{eq:gamupdate}, we have
\[
    \eta_\ell=\gamma^+_\ell + \gamma^-_\ell = \frac{\gamma^+_\ell}{\alpha_\ell^-} =
     \frac{\gamma_\ell^-}{\alpha_\ell^+}.
\]
Therefore,
\beq\label{eq:alphaone}
    \alpha_\ell^- = \frac{\gamma^+_\ell}{\gamma_\ell^++\gamma_\ell^-}
        = 1- \frac{\gamma^-_\ell}{\gamma_\ell^++\gamma_\ell^-} = 1-\alpha^+_\ell.
\eeq
% Hence,
% \beq \label{eq:alphaone}
%     \alpha^+_\ell + \alpha^-_\ell = 1.
% \eeq
Now, from line~\ref{line:rp} in Algorithm~\ref{algo:ml-vamp},
\begin{align}
     \zbfhat^+_\ell &= (1-\alpha^+_\ell)\rbf^+_\ell + \alpha^+_\ell\rbf^-_\ell \nonumber \\
       & = \alpha^-_\ell\rbf^+_\ell + \alpha^+_\ell\rbf^-_\ell, \label{eq:zhatfix1}
\end{align}
where the last step used \eqref{eq:alphaone}.  Similarly, from line~\ref{line:rn},
\beq
    \zbfhat^-_\ell = \alpha^-_\ell\rbf^+_\ell + \alpha^+_\ell\rbf^-_\ell. \label{eq:zhatfix2}
\eeq
Equations \eqref{eq:zhatfix1} and \eqref{eq:zhatfix2} prove \eqref{eq:zcon}.
In the sequel, we will let $\zbfhat_\ell$ denote $\zbfhat^+_\ell$ and $\zbfhat^-_\ell$
since they are equal. As a consequence of the primal feasibility $\zbfhat^+_\ell=\zbfhat^-_\ell$, observe that
\beq
\sbf_\ell^+-\sbf_\ell^- = (\alpha_\ell^++\alpha_\ell^-)\zbfhat_\ell - \alpha^+_\ell\rbf_\ell^--\alpha^-_\ell\rbf_\ell^+=0,
\eeq
where we have used \eqref{eq:alphaone} and \eqref{eq:zhatfix1}. Define $\sbf:=\sbf^+=\sbf^-$, by virtue of the equality shown above.

Having shown the equivalence of Algorithm \ref{algo:ml-vamp} and the iterative updates in the statement of the theorem, we can say that there exists a one-to-one linear mapping between their fixed points $\{\zbfhat,\rbf^{+},\rbf^{-}\}$ (from Algorithm \ref{algo:ml-vamp}) and $\{\zbfhat,\sbf\}$ (from Theorem \ref{thm:mapfix}). Now to show \eqref{eq:Laggrad} it suffices to show that $\sbf_\ell$ is a valid dual parameter for which the following stationarity conditions hold,
\begin{align} \label{eq:Laggrad_l}
    \frac{\partial \mc L_\ell(\zbf^-_{\ell-1},\zbf^+_{\ell};\zbfhat^+_{\ell-1},\zbfhat^-_{\ell},\sbf_{\ell-1},\sbf_{\ell})}{\partial \zbf^-_{\ell-1}}\Bigg{\rvert}_{(\zbfhat_{\ell-1}^-,\zbfhat_{\ell}^+)}\owns\ &\ {\bf 0}, \\
    \frac{\partial \mc L_\ell(\zbf^-_{\ell-1},\zbf^+_{\ell};\zbfhat^+_{\ell-1},\zbfhat^-_{\ell},\sbf_{\ell-1},\sbf_{\ell})}{\partial \zbf^+_\ell}\Bigg{\rvert}_{(\zbfhat_{\ell-1}^-,\zbfhat_{\ell}^+)}\owns\ &\ {\bf 0}.
\end{align}
Indeed the above conditions are the stationarity conditions of the optimization problem in \eqref{eq:admmHp} and \eqref{eq:admmHn}.



\section{Empirical Convergence of Random Variables} \label{sec:empirical}

We follow the framework of Bayati and Montanari \citep{BayatiM:11}, which models
various sequences as deterministic, but with components converging empirically
to a distribution.  We start with a brief review of useful definitions.
Let $\xbf = (\xbf_1,\ldots,\xbf_N)$ be a block vector with components $\xbf_n \in \R^r$
for some $r$.  Thus, the vector $\xbf$
is a vector with dimension $rN$.
Given any function $g:\R^r \arr \R^s$, we define the
\emph{componentwise extension} of $g(\cdot)$ as the function,
\beq \label{eq:gcomp}
    \gbf(\xbf) := (g(\xbf_1),\ldots,g(\xbf_N)) \in \R^{Ns}.
\eeq
That is,
$\gbf(\cdot)$
applies the function
$g(\cdot)$
on each $r$-dimensional component.
Similarly,
we say $\gbf(\xbf)$ \emph{acts componentwise} on $\xbf$ whenever it is of the form \eqref{eq:gcomp}
for some function $g(\cdot)$.

Next consider a sequence of block vectors of growing dimension,
\[
    \xbf(N) = (\xbf_1(N),\ldots,\xbf_N(N)),
\qquad
N=1,\,2,\,\ldots,
\]
where each component $\xbf_n(N) \in \R^r$.
In this case, we will say that
$\xbf(N)$ is a \emph{block vector sequence that scales with $N$
under blocks $\xbf_n(N) \in \R^r$.}
When $r=1$, so that the blocks are scalar, we will simply say that
$\xbf(N)$ is a \emph{vector sequence that scales with $N$}.
Such vector sequences can be deterministic or random.
In most cases, we will omit the notational dependence on $N$ and simply write $\xbf$.

Now, given $p \geq 1$,
a function $f:\R^r \arr \R^s$ is called \emph{pseudo-Lipschitz continuous of order $p$},
if there exists a constant $C > 0$ such that for all $\xbf_1,\xbf_2 \in\R^r$,
\[
    \| f(\xbf_1)- f(\xbf_2) \| \leq C\|\xbf_1-\xbf_2\|\left[ 1 + \|\xbf_1\|^{p-1}
    + \|\xbf_2\|^{p-1} \right].
\]
Observe that in the case $p=1$, pseudo-Lipschitz continuity reduces to
the standard Lipschitz continuity.
Given $p \geq 1$, we will say that the block vector sequence $\xbf=\xbf(N)$
\emph{converges empirically with $p$-th order moments} if there exists a random variable
$X \in \R^r$ such that
\begin{enumerate}[(i)]
\item $\Exp\|X\|_p^p < \infty$; and
\item for any $f : \R^r \arr \R$ that is pseudo-Lipschitz continuous of order $p$,
\beq \label{eq:PLp-empirical}
    \lim_{N \arr \infty} \frac{1}{N} \sum_{n=1}^N f(\xbf_n(N)) = \Exp\left[ f(X) \right].
\eeq
\end{enumerate}
In \eqref{eq:PLp-empirical}, we have
the empirical mean of the components $f(\xbf_n(N))$
of the componentwise extension $\fbf(\xbf(N))$
converging to the expectation $\Exp[ f(X) ]$.
In this case, with some abuse of notation, we will write
\beq \label{eq:plLim}
    \lim_{N \arr \infty} \left\{ \xbf_n \right\} \stackrel{PL(p)}{=} X,
\eeq
where, as usual, we have omitted the dependence on $N$ in $\xbf_n(N)$.
Importantly, empirical convergence can de defined on deterministic vector sequences,
with no need for a probability space.  If $\xbf=\xbf(N)$ is a random vector sequence,
we will often require that the limit \eqref{eq:plLim} holds almost surely.

We conclude with one final definition.
Let $\phibf(\rbf,\gamma)$ be a function on $\rbf \in \R^s$ and $\gamma \in \R$.
We say that $\phibf(\rbf,\gamma)$ is \emph{uniformly Lipschitz continuous} in $\rbf$
at $\gamma=\gammabar$ if there exists constants
$L_1$ and $L_2 \geq 0$ and an open neighborhood $U$ of $\gammabar$, such that
\beq \label{eq:unifLip1}
    \|\phibf(\rbf_1,\gamma)-\phibf(\rbf_2,\gamma)\| \leq L_1\|\rbf_1-\rbf_2\|,
\eeq
for all $\rbf_1,\rbf_2 \in \R^s$ and $\gamma \in U$; and
\beq \label{eq:unifLip2}
    \|\phibf(\rbf,\gamma_1)-\phibf(\rbf,\gamma_2)\| \leq L_2\left(1+\|\rbf\|\right)|\gamma_1-\gamma_2|,
\eeq
for all $\rbf \in \R^s$ and $\gamma_1,\gamma_2 \in U$.

\section{Large System Limit: Model Details} \label{sec:lsl}

In addition to the assumptions in Section~\ref{sec:seevo},
we describe a few more technical assumptions.
First, we need that the activation functions
$\phibf_\ell(z_{\lm1},\xi_\ell)$ in \eqref{eq:nnnonlintrue} act \emph{componentwise} meaning
that,
\beq \label{eq:phicomp}
 \left[ \phibf_{\ell}(\zbf_{\lm1}, \xibf_\ell) \right]_n
    = \phi_\ell(z_{\lm1,n},\xi_{\ell,n})
\eeq
for some scalar-valued function $\phi_\ell(\cdot)$ for all components $n$. That is, for a nonlinear layer
$\ell=2,4,\ldots,L$, each output $z^0_{\ell,n}$ depends only on the corresponding input component
$z^0_{\lm1,n}$.  Standard activations such as ReLU or sigmoid would satisfy this property.
In addition, we require that the activation function components $\phi_\ell(\cdot)$
are pseudo-Lipschitz continuous of order two.

Next, we
need certain assumptions on the estimation functions $\gbf_\ell^{\pm}(\cdot)$.
For the estimation functions corresponding to the  nonlinear layers,
$\ell=2,4,\ldots,L-2$, we assume that for each parameter $\theta_{k\ell}^-$, the function
$\gbf_\ell^+(\rbf_{\lm1}^+,\rbf_{\ell}^-,\theta_{\ell}^-)$ is Lipschitz
continuous in $(\rbf^+_{\lm1},\rbf^-_\ell)$ and $\gbf^+_\ell(\cdot)$ acts
\emph{componentwise} in that,
\beq \label{eq:gprow}
    \zbfhat^+_\ell = \gbf_\ell^+(\rbf^+_{\lm1},\rbf^-_\ell,\theta_\ell^+)
    \Leftrightarrow
    \zhat^+_{\ell,i} = g_\ell^+(r^+_{\lm1,i},r^-_{\ell,i},\theta_\ell^+),
\eeq
for $i=1,\ldots,N_\ell$.
for some scalar-valued function $g_\ell^+(\cdot)$. Thus, each element
$\zhat^+_{\ell,i}$ of the output vector $\zbfhat^+_\ell$ depends only the corresponding elements of the inputs
$r^+_{\lm1,i}$ and $r^-_{\ell,i}$.  We make a similar assumption on the first estimation function
$\gbf^+_0(\cdot)$ as well as the reverse functions $\gbf^-_\ell(\cdot)$ for $\ell=2,4,\ldots,L$ and define $g_0^+(\cdot)$ and $g_\ell^-(\cdot)$ in a similar manner.

Note that for the linear layers $\ell=1,3,\ldots,\Lm1$, we assume the MAP denoiser \eqref{eq:gmap}.
For the linear layer, this is identical to the MMSE denoiser and the estimation functions can be written as,
\begin{subequations}\label{eq:glintrans}
\begin{align}
  \MoveEqLeft \gbf^+_\ell(\rbf^+_{\lm1},\rbf^-_{\lm1},\theta^+_{\ell}) \nonumber \\
  &=
  \Vbf_\ell{\Gbf}^+_\ell(\Vbf_{\lm1}\rbf^+_{\lm1},\Vbf_{\ell}\tran\rbf^-_{\lm1},
  \bar{\sbf}_\ell,\bar{\bbf}_\ell,\theta^-_{\ell}) \\
  \MoveEqLeft \gbf^-_\ell(\rbf^+_{\lm1},\rbf^-_{\lm1},\theta^+_{\ell}) \nonumber \\
   &:=
  \Vbf_{\lm1}\tran{\Gbf}^+_\ell(\Vbf_{\lm1}\rbf^+_{\lm1},\Vbf_{\ell}\tran\rbf^-_{\lm1},
  \bar{\sbf}_\ell,\bar{\bbf}_\ell,   \theta^-_{\ell}),
\end{align}
\end{subequations}
where, for each parameter value $\theta^{\pm}_\ell$, the functions ${\Gbf}^{\pm}_\ell(\cdot)$ are Lipschitz continuous in
$(\rbf^+_{\lm1},\rbf^-_\ell,\bar{\sbf}_\ell)$ and are componentwise extensions of ${G}_\ell^{\pm}$ defined as,
\begin{align}
    \MoveEqLeft \begin{bmatrix}
        {G}_\ell^-(\bar{u}_{\lm1},\bar{u}_\ell,s_\ell,\bar{b}_\ell,\gamma_{\lm1}^+,\gamma_{\ell}^-) \\
        {G}_\ell^+(\bar{u}_{\lm1},\bar{u}_\ell,s_\ell,\bar{b}_\ell,\gamma_{\lm1}^+,\gamma_{\ell}^-)
    \end{bmatrix}
    \nonumber \\
       & =  \begin{bmatrix}
        \gamma_{\lm1}^+ + \nu_\ell s_\ell^2 & -\nu_\ell s_\ell \\
        -\nu_\ell s_\ell & \gamma_\ell^- +\nu_\ell
        \end{bmatrix}^{-1}
        \begin{bmatrix}
        \gamma_{\lm1}^+ \bar{u}_{\lm1} - \nu_\ell s_\ell \bar{b}_\ell \\
        \gamma_{\ell}^- \bar{u}_{\ell} + \nu_\ell \bar{b}_\ell
        \end{bmatrix}, \label{eq:gdeflin}
\end{align}
We call the functions ${\Gbf}^{\pm}_\ell(\cdot)$, the \emph{transformed denoising
functions}. We refer the reader to the appendices
of \cite{fletcher2017inference} for a detailed derivation of $\Gbf^{\pm}_\ell$.
We now need two further technical assumptions.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]
\caption{Transformed ML-VAMP Recursion}
\begin{algorithmic}[1]  \label{algo:trans}
\STATE{// Initialization }
\STATE{Initial vectors $\wbf_\ell$, $\qbf^0_0$, $\qbf_{0\ell}^-$}
    \label{line:init_gen}
\STATE{$\qbf^0_0 = \fbf^0_0(\wbf_0), \quad \pbf^0_0 = \Vbf_0\qbf^0_0$} \label{line:q00init_gen}
\FOR{$\ell=1,\ldots,\Lm1$}
    \STATE{$\qbf^0_\ell = \fbf^0_\ell(\pbf^0_{\lm1},\wbf_\ell, \Lambda_{01}^-)$ }
    \label{line:q0init_gen}
    \STATE{$\pbf^0_\ell = \Vbf_\ell\qbf^0_\ell$ }  \label{line:p0init_gen}
\ENDFOR
%\STATE{Initialize parameter list:  $\Lambda_{01}^-$} \label{line:laminit_gen}
%\STATE{Initialize vectors:  $\qbf_{0\ell}^-$, $\ell=0,\ldots,\Lm1$} \label{line:qinit_gen}
\STATE{}

\FOR{$k=0,1,\dots,N_{\rm it}-1$}

    \STATE{// Forward Pass }
    \STATE{$\qbfhat^+_{k0} = \hbf^+_0(\qbf^-_{k\ell},\wbf_\ell,\theta^+_{k0})$ }
    \STATE{$\alpha^+_{k0} = \bkt{\partial
        \hbf^+_0(\qbf^-_{k0},\wbf_\ell,\theta^+_{k0})/\partial \qbf^-_{k0}}$}
        \label{line:alphagenp0}
    \STATE{$\Lambda_{k0}^+ = (\alpha_{k0}^+,\theta_{k0}^+)$}
    \STATE{$\qbf^+_{k0} = \fbf^+_0(\qbf^-_{k0},\wbf_\ell,\Lambda^+_{k0})$ }
    \STATE{$\pbf^+_{k0} = \Vbf_0 \qbf^+_{k0}$}
    \FOR{$\ell=1,\ldots,\Lm1$}
        \STATE{$\qbfhat^+_{k\ell} = \hbf^+_\ell(\pbf^0_{\lm1},\pbf^+_{k,\lm1},
            \qbf^-_{k\ell},\wbf_\ell,\theta^+_{k\ell})$ }
        \STATE{$\alpha^+_{k\ell} = \bkt{\partial
            \hbf^+_\ell(\pbf^+_{k,\lm1},\qbf^-_{k\ell},\wbf_\ell,\theta^+_{k\ell})/\partial \qbf^-_{k\ell}}$}
            \label{line:alphagenp}
        \STATE{$\Lambda_{k\ell}^+ = (\alpha_{k\ell}^+,\theta_{k\ell}^+)$}
        \STATE{$\qbf^+_{k\ell} = \fbf^+_\ell(\pbf^+_{k,\lm1},\qbf^-_{k\ell},\wbf_\ell,
            \Lambda^+_{k\ell})$ }
        \STATE{$\pbf^+_{k\ell} = \Vbf_\ell \qbf^+_{k\ell}$}
    \ENDFOR
    \STATE{}

    \STATE{// Reverse Pass }
    \STATE{$\pbfhat^-_{\kp1,\Lm1} =
        \hbf^-_{L}(\pbf^+_{k,\Lm1},\wbf_{L},\theta^-_{kL})$ }
    \STATE{$\alpha^-_{k,\Lm1} = \bkt{\partial
        \hbf^-_{L}(\pbf^+_{k,\Lm1},\wbf_{L},
        \theta^-_{kL})/\partial \pbf^+_{k,\Lm1}}$}
        \label{line:alphagennL}
    \STATE{$\Lambda_{kL}^- = (\alpha_{k,\Lm1}^-,\theta_{kL}^-)$}
    \STATE{$\pbf^-_{\kp1,\Lm1} =
        \fbf^-_{L}(\pbf^+_{k,\Lm1},\wbf_{L},\Lambda^-_{kL})$ }
    \FOR{$\ell=L-2,\ldots,0$}
        \STATE{$\pbfhat^-_{\kp1,\lm1} = \hbf^-_{\lp1}(\pbf^+_{k\ell},\qbf^-_{k,\lp1},\wbf_{\lp1},\theta^-_{k,\lp1})$}
        \STATE{$\alpha^-_{k\ell} =
        \bkt{\partial \hbf^-_{\lp1}(\pbf^+_{k\ell},\cdots)/\partial \pbf^+_{k\ell}}$}
            \label{line:alphagenn}
        \STATE{$\Lambda_{k,\lp1}^- = (\alpha_{k,\lp1}^-,\theta_{k,\lp1}^-)$}
        \STATE{$\pbf^-_{\kp1,\ell} =
            \fbf^-_{\lp1}(\pbf^+_{k\ell},\qbf^-_{k,\lp1},\wbf_{\lp1},\Lambda^-_{k,\lp1})$ }
        \STATE{$\qbf^-_{\kp1,\ell} = \Vbf_\ell\tran \pbf^-_{\kp1,\ell}$}
    \ENDFOR

\ENDFOR
\end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]
\caption{State Evolution for ML-VAMP}
\begin{algorithmic}[1]  \label{algo:gen_se}

\REQUIRE{Vector update component functions $f^0_\ell(\cdot)$ and $f^\pm_{k\ell}(\cdot)$}

\STATE{}
\STATE{// Initial pass}
\STATE{Initial random variables:  $W_\ell$, $Q_{0\ell}^-$, $\ell=0,\ldots,\Lm1$}
    \label{line:qinit_se_gen}
\STATE{$Q^0_0 = f^0_0(W_0)$} \label{line:q0init_se_gen}
\STATE{$P^0_0 \sim \Norm(0,\tau^0_0)$, $\tau^0_0 = \Exp(Q^0_0)^2$} \label{line:p0init_se_gen}
\FOR{$\ell=1,\ldots,\Lm1$}
    \STATE{$Q^0_\ell=f^0_\ell(P^0_{\lm1},W_\ell)$}
    \STATE{$P^0_\ell = \Norm(0,\tau^0_\ell)$,
            $\tau^0_\ell = \Exp(Q^0_\ell)^2$} \label{line:pinit_se_gen}
\ENDFOR
\STATE{}

\FOR{$k=0,1,\dots$}
    \STATE{// Forward Pass }
    %\STATE{$\lambdabar^+_{k0} = T_{k0}^+(\mubar^+_{k0},\Lambdabar_{0k}^-), \quad
    %    \mubar^+_{k0} = \Exp(\varphi_{k0}^+(Q_{k0}^-,W_0,\Lambdabar_{0k}^-))$}    \label{line:mup0_se_gen}
    %\STATE{$\Lambdabar_{k0}^+ = (\Lambdabar_{k1}^-,\lambdabar^+_{k0})$} \label{line:lamp0_se_gen}
    \STATE{$\hat{Q}^+_{k0} = h^+_0(Q_{k0}^-,W_0,\theta^+_{k0}))$} \label{line:qhat0_se_gen}
    \STATE{$\alphabar_{k0}^+ = \Exp(\partial h^+_0(Q_{k0}^-,W_0,\theta^+_{k0})/\partial Q_{k0}^-)$}
    \STATE{$\Lambdabar_{k0}^+ = (\alphabar^+_{k0},\theta_{k0}^+)$}
    \STATE{$Q_{k0}^+ = f^+_{k0}(Q_{k0}^-,W_0,\Lambdabar^+_{k0})$}  \label{line:q0_se_gen}
    \STATE{$(P^0_0,P_{k0}^+) = \Norm(\zero,\Kbf_{k0}^+)$,
        $\Kbf_{k0}^+ = \Cov(Q^0_0,Q_{k0}^+)$} \label{line:p0_se_gen}
    \FOR{$\ell=1,\ldots,L-1$}
        \STATE{$\hat{Q}^+_{k\ell} = h^+_\ell(P^0_{\lm1},P^+_{k,\lm1},Q_{k\ell}^-,
            W_\ell,\theta^+_{k\ell}))$} \label{line:qhat_se_gen}
        \STATE{$\alphabar_{k0}^+ = \Exp(\partial h^+_\ell(\ldots))/\partial Q_{k\ell}^-)$}
        \STATE{$\Lambdabar_{k\ell}^+ = (\alphabar^+_{k\ell},\theta_{k\ell}^+)$}
            \label{line:lamp_se_gen}
        \STATE{$Q_{k\ell}^+ = f^+_{k\ell}(P^0_{\lm1},P^+_{k,\lm1},Q_{k\ell}^-,W_\ell,\Lambdabar^+_{k\ell})$}
            \label{line:qp_se_gen}
        \STATE{$(P^0_\ell,P_{k\ell}^+) = \Norm(\zero,\Kbf_{k\ell}^+)$,
            $\Kbf_{k\ell}^+ = \Cov(Q^0_\ell,Q_{k\ell}^+) $}   \label{line:pp_se_gen}
    \ENDFOR
    \STATE{}

    \STATE{// Reverse Pass }
    \STATE{$\hat{P}_{\kp1,\Lm1}^- = h^-_{kL}(P^0_{\Lm1},P_{k,\Lm1}^+,W_L,\theta^-_{\kp1,L})$}
        \label{line:phatL_se_gen}
    \STATE{$\alphabar_{k,\Lm1}^- = \partial h^-_{kL}(\cdots)/  \partial P_{k,\Lm1}^+$}
    \STATE{$\Lambdabar_{k,\Lm1}^- = (\alphabar^-_{k,\Lm1},\theta_{k,\Lm1}^-)$}
    \STATE{$P_{\kp1,\Lm1}^- = f^-_{kL}(P^0_{\Lm1},P_{k,\Lm1}^+,W_L,\Lambdabar^-_{\kp1,L})$}  \label{line:pL_se_gen}
    \STATE{$\tau_{\kp1,\Lm1}^- = \Exp(P^-_{\kp1,\Lm1})^2$} \label{line:tauL_se_gen}
    \STATE{$Q_{\kp1,\Lm1}^- = \Norm(0,\tau_{\kp1,\Lm1}^-)$} \label{line:qL_se_gen}
    \FOR{$\ell=\Lm1,\ldots,1$}
        \STATE{$\hat{P}_{\kp1,\lm1}^- = h^-_{k\ell}(P^0_{\lm1},P_{k,\lm1}^+,W_\ell,\theta^-_{\kp1,\ell})$}
            \label{line:phatn_se_gen}
        \STATE{$\alphabar_{k,\lm1}^- = \Exp(\partial h^-_{k\ell}(\ldots)/ \partial P_{k,\Lm1}^+)$}
        \STATE{$\Lambdabar_{k\ell}^- = (\alphabar^-_{k,\lm1},\theta_{k,\ell}^-)$}
       \STATE{$P_{\kp1,\lm1}^- =
        f^-_{k\ell}(P^0_{\lm1},P^+_{k,\lm1},Q_{\kp1,\ell}^-,W_\ell,\Lambdabar^-_{k\ell})$}
            \label{line:pn_se_gen}
        \STATE{$\tau_{\kp1,\lm1}^- = \Exp(P_{\kp1,\lm1}^-)^2$} \label{line:taun_se_gen}
        \STATE{$Q_{\kp1,\lm1}^- = \Norm(0,\tau_{\kp1,\lm1}^-)$}   \label{line:qn_se_gen}
    \ENDFOR

\ENDFOR
\end{algorithmic}
\end{algorithm}



\section{Proof of Theorem \ref{thm:mapse}}  \label{sec:mapsepf}

\subsection{Transformed MLP}

The SE analysis of MMSE ML-VAMP in \cite{fletcher2017inference} proves a result on
a general class of multi-layer recursions, called Gen-ML.  To prove Theorem~\ref{thm:mapse},
we will show that ML-VAMP algorithm in Algorithm~\ref{algo:ml-vamp} is of the form
of an almost identical recursion with some minor changes in notation.
Theorem~\ref{thm:mapse} in this paper
will then follow from applying the general result in
\cite{fletcher2017inference}.  Since most of the proof is identical, we highlight only the
main differences.

Similar to \cite{fletcher2017inference}, we rewrite the MLP in \eqref{eq:nntrue} in
a certain transformed form.  To this end, define the disturbance vectors,
\begin{subequations} \label{eq:wdef}
\begin{align}
    \wbf_0 &:= \zbfhat^0_0, \quad
    \wbf_{\ell} := \xibf_\ell, \quad \ell =2,4,\ldots,L \\
    \wbf_{\ell} &= (\bar{\sbf}_{\ell},\bar{\bbf}_\ell,\bar{\xibf}_\ell),  \quad \ell =1,3,\ldots,\Lm1.
\end{align}
\end{subequations}
Also, define the scalar-valued functions,
\begin{subequations} \label{eq:f0ml}
\begin{align}
    \MoveEqLeft f^0_0(w_0) := w_0, \\
    \MoveEqLeft f^0_\ell(p^0_{\lm1},w_\ell) = f^0_\ell(p^0_{\lm1},\xi_\ell) := \phi_\ell(p^0_{\lm1},\xi_\ell), \nonumber \\
    & \ell=2,4,\ldots,L    \label{eq:f0nonlin} \\
    \MoveEqLeft f^0_\ell(p^0_{\lm1},w_\ell) = f^0_\ell(p^0_{\lm1},(\bar{s}_\ell,\bar{b}_\ell,\bar{\xi}_\ell))
        = \bar{s}_\ell p^0_\ell + \bar{b}_\ell + \bar{\xi}_\ell, \nonumber \\
    & \ell=1,3,\ldots,\Lm1.    \label{eq:f0lin}
\end{align}
\end{subequations}
Let $\fbf^0_\ell(\cdot)$ be their \emph{componentwise extension}, meaning that
\[
    \left[ \fbf^0_\ell(\pbf^0_{\lm1,n},\wbf_{\ell,n})\right]_n
    := f^0_\ell(p^0_{\lm1,n},w_{\ell,n}),
\]
so that $\fbf^0_\ell(\cdot)$ acts with the scalar-valued function $f^0_\ell(\cdot)$ on
each component of the vectors.
With this definition, it is shown in \cite{fletcher2017inference} that
the vectors $\pbf^0_\ell$ and $\qbf^0_\ell$ satisfy the recursions in
``Initialization" section of Algorithm~\ref{algo:trans}, the transformed algorithm.
This system of equations is represented diagrammatically in
the top panel of Fig.~\ref{fig:transformed}.
In comparison to Fig.~\ref{fig:nn_ml_vamp}, the transforms $\Wbf_\ell$ of the linear
 layers have been expanded using the SVD $\Wbf_{\ell} = \Vbf_{\ell}\Sigmabf_\ell\Vbf_{\lm1}$
 and inserting intermediate variables $\qbf^0_\ell$ and $\pbf^0_\ell$.
With the transformation, the  MLP \eqref{eq:nntrue} is equivalent to
a sequence of linear transforms by orthogonal matrices $\Vbf_\ell$ and non-linear componentwise
mappings $f^0_\ell(\cdot)$.



\begin{figure*}
\begin{tikzpicture}

    \tikzstyle{var}=[draw,circle,fill=green!20,node distance=2.5cm]
    \tikzstyle{linblock}=[draw,fill=blue!20, minimum size=1cm, node distance=2cm];
    \tikzstyle{nlblock}=[draw,fill=green!20, minimum size=1cm, node distance=2cm];
    \tikzstyle{vblock}=[draw,fill=purple!10, minimum size=1cm, node distance=2cm];

    \node [nlblock] (z0) {$\fbf^0_0$};
    \node [vblock, right of=z0] (V0) {$\Vbf_0$};
    \node [linblock, right of=V0] (S1) {$\fbf^0_1$};
    \node [vblock, right of=S1] (V1) {$\Vbf_1$};
    \node [nlblock, right of=V1] (phi2) {$\fbf^0_2$};
    \node [vblock, right of=phi2] (V2) {$\Vbf_2$};
    \node [linblock, right of=V2] (S3) {$\fbf^0_3$};
    \node [vblock, right of=S3] (V3) {$\Vbf_3$};
    \node [var, right of=V3] (phi4) {};
    %\node [right of=phi4, node distance=2cm] (y) {};

    \node [nlblock,below of=z0] (h0) {$\fbf_0^+$};
    \node [vblock, below of=V0] (V0b) {$\Vbf_0$};
    \node [linblock, below of=S1] (h1) {$\fbf_1^{\pm}$};
    \node [vblock, below of=V1] (V1b) {$\Vbf_1$};
    \node [nlblock, below of=phi2] (h2) {$\fbf_2^{\pm}$};
    \node [vblock, below of=V2] (V2b) {$\Vbf_2$};
    \node [linblock, below of=S3] (h3) {$\fbf_3^{\pm}$};
    \node [vblock, below of=V3] (V3b) {$\Vbf_3$};
    \node [nlblock, below of=phi4] (h4) {$\fbf_4^-$};


    % Draw arrows
    \path[->] (z0) edge  node [above] {{\begin{tabular}{l} $\zbf^0_0=$ \\ $\qbf^0_0$ \end{tabular}}} (V0);
    \path[->] (V0) edge  node [above] {$\pbf^0_0$} (S1);
    \path[->] (S1) edge  node [above] {$\qbf_1^0$} (V1);
    \path[->] (V1) edge  node [above] {{\begin{tabular}{l} $\zbf^0_1=$ \\ $\pbf^0_1$ \end{tabular}}} (phi2);
    \path[->] (phi2) edge  node [above] {{\begin{tabular}{l} $\zbf^0_2=$ \\ $\qbf^0_2$ \end{tabular}}} (V2);
    \path[->] (V2) edge  node [above] {$\pbf^0_2$} (S3);
    \path[->] (S3) edge  node [above] {$\qbf^0_3$} (V3);
    \path[->] (V3) edge  node [above] {{\begin{tabular}{l} $\zbf^0_3=$ \\ $\pbf^0_3$ \end{tabular}}} (phi4);

    \path[<->] (h0) edge  node [above]
        {{\begin{tabular}{c} $\rbf^{\pm}_{k0}-\zbf^0_0$ \\ $\qbf^{\pm}_{k0}$ \end{tabular}}} (V0b);
    \path[<->] (V0b) edge  node [above] {$\pbf^{\pm}_{k0}$} (h1);
    \path[<->] (h1) edge  node [above] {$\qbf^{\pm}_{k1}$} (V1b);
    \path[<->] (V1b) edge  node [above]
        {{\begin{tabular}{c} $\rbf^{\pm}_{k1}-\zbf^0_1$ \\ $\pbf^{\pm}_{k1}$ \end{tabular}}}  (h2);
    \path[<->] (h2) edge  node [above]
        {{\begin{tabular}{c} $\rbf^{\pm}_{k2}-\zbf^0_2$ \\ $\qbf^{\pm}_{k2}$ \end{tabular}}} (V2b);
    \path[<->] (V2b) edge  node [above] {$\pbf^{\pm}_{k2}$} (h3);
    \path[<->] (h3) edge  node [above] {$\qbf^{\pm}_{k3}$} (V3b);
    \path[<->] (V3b) edge  node [above]
        {{\begin{tabular}{c} $\rbf^{\pm}_{k3}-\zbf^0_3$ \\ $\pbf^{\pm}_{k3}$ \end{tabular}}} (h4);
\end{tikzpicture}
\caption{Transformed view of the MLP and message passing system in Fig.~\ref{fig:nn_ml_vamp}.
The linear transforms $\Wbf_\ell$ are replaced by the SVD $\Wbf_\ell = \Vbf_\ell\Sigmabf_\ell\Vbf_{\lm1}$,
and intermediate layers are added for each component of the SVD.  With this transformation,
the MLP and message passing algorithm are reduced to alternating multiplications by $\Vbf_\ell$ and $\Vbf_\ell^*$
and componentwise (possibly nonlinear) functions.
 \label{fig:transformed}}
\end{figure*}

\subsection{Parameters}
To handle parameterized functions, the analysis in \cite{fletcher2017inference} introduces
the concept of \emph{parameter lists}.  For our purpose, let
\beq \label{eq:lamlist}
    \Lambda^+_{k\ell} := (\alpha_{k\ell}^+,\theta_{k\ell}^+), \quad
    \Lambda^-_{k\ell} := (\alpha_{k\ell}^-,\theta_{k\ell}^-),
\eeq
which is simply the parameter $\alpha_{k\ell}^{\pm}$ along with the parameter $\theta_{k\ell}^{\pm}$
for the estimators.

\subsection{Estimation Functions}
Similar to the transformed system in the top panel of Fig.~\ref{fig:transformed},
we next represent the steps in the
ML-VAMP Algorithm~\ref{algo:ml-vamp} as a sequence of alternating linear and nonlinear maps.
Let $\ell=0,2,4,\ldots,L$ be the index of  a nonlinear layer and
define the scalar-valued functions,
\begin{subequations} \label{eq:hnonlin}
\begin{align}
    \MoveEqLeft h^{+}_{0}(q_{0}^-,w_0,\theta_{k0}^+)
        := g^{+}_0(q^-_0 + w_0,\theta_{k0}^+), \label{eq:gtp0nonlin} \\
    \MoveEqLeft h^{+}_{\ell}(p^0_{\lm1},p_{\lm1}^+,q_{\ell}^-,w_\ell,\theta_{k\ell}^+) \nonumber \\
        &:= g^{+}_\ell(p_{\lm1}^+ +p^0_{\lm1},q^-_\ell + q^0_\ell,\theta_{k\ell}^+),  \label{eq:hpnonlin} \\
    \MoveEqLeft h^{-}_{L}(p^0_{\Lm1},p_{\Lm1}^+,w_L,\theta_{k,L}^-)
        := g^{-}_L(p_{\Lm1}^+ + p^0_{\Lm1},\theta_{k,L}^-). \label{eq:gtnLnonlin} \\
    \MoveEqLeft h^{-}_{\ell}(p^0_{\lm1},p_{\lm1}^+,q_{\ell}^-,w_\ell,\theta_{k,\lp1}^+) \nonumber \\
        &:= g^{-}_\ell(p_{\lm1}^+ +p^0_{\lm1},q^-_\ell + q^0_\ell,\theta_{k\ell}^-), \label{eq:hnnonlin}
\end{align}
\end{subequations}
For $\ell=1,3,\ldots,\Lm1$, the index of a linear layer, and
$w_\ell=(\bar{s}_\ell,\bar{b}_\ell)$, let
\begin{subequations} \label{eq:hlin}
\begin{align}
    \MoveEqLeft
    h^{+}_{\ell}(p_{\lm1}^0,p_{\lm1}^+,q_{\ell}^-,w_\ell,\theta_{k\ell}^+) \nonumber \\
        &:=  G^{+}_\ell(p_{\lm1}^+ +p^0_{\lm1},q^-_\ell + q^0_\ell, \bar{s}_\ell, \bar{b}_\ell,
        \theta^+_{k\ell}), \label{eq:hplin} \\
    \MoveEqLeft
    h^{-}_{\ell}(p_{\lm1}^0,p_{\lm1}^+,q_{\ell}^-,w_\ell,\theta_{k\ell}^-) \nonumber \\
        &:= G^{-}_\ell(p_{\lm1}^+ +p^0_{\lm1},q^-_\ell + q^0_\ell, \bar{s}_\ell, \bar{b}_\ell,
            \theta^-_{k\ell}), \label{eq:hnlin}
\end{align}
\end{subequations}
where $G^{\pm}(\cdot)$ are the components of the transformed linear estimation functions.
%Then, for all $\ell$,
%\begin{subequations} \label{eq:hnonlin}
%\begin{align}
%    \MoveEqLeft h^{+}_{k0}(q_{0}^-,w_0,\theta_{k0}^+)
%        := \tilde{g}^{+}_0(q^-_0,w_0,\theta_{k0}^+)
%        - w^0_\ell. \label{eq:hp0nonlin} \\
%    \MoveEqLeft h^{+}_{k\ell}(p^0_{\lm1},p_{\lm1}^+,q_{\ell}^-,w_\ell,\theta_{k\ell}^+) \nonumber \\
%        &:=\tilde{g}^{+}_{k\ell}(p^0_{\lm1},p_{\lm1}^+,q_{\ell}^-,w_\ell,\theta_{k\ell}^+)
%        - q^0_\ell,  \label{eq:hpnonlin} \\
%    \MoveEqLeft h^{-}_{kL}(p^0_{\Lm1},p_{\Lm1}^+,w_L,\theta_{k,L}^-) \nonumber \\
%        &:= \tilde{g}^{-}_{kL}(p^0_{\Lm1},p_{\Lm1}^+,w_L,\theta_{k,L}^-)  -
%            p^0_{\lm1}. \label{eq:hnLnonlin} \\
%    \MoveEqLeft h^{-}_{k\ell}(P^0_{\lm1},P_{\lm1}^+,Q_{\ell}^-,W_\ell,\theta_{k,\lp1}^+) \nonumber \\
%        &:= \tilde{g}^{-}_{k\ell}(p^0_{\lm1},p_{\lm1}^+,q_{\ell}^-,w_\ell,\theta_{k,\lp1}^+)
%        - p^0_{\lm1}, \label{eq:hnnonlin}
%\end{align}
%\end{subequations}
For both the linear and nonlinear layers, we then define the update functions as,
\begin{subequations} \label{eq:fhdef}
\begin{align}
    \MoveEqLeft f^{+}_{0}(q_{0}^-,w_0,\Lambda_{k0}^+) := \frac{1}{1-\alpha_{k\ell}^+} \nonumber \\
     &\times \left[
            h^{+}_{0}(q_{0}^-,w_0,\theta_{k0}^+) -w_0
            - \alpha_{k0}^+ q_0^- \right], \label{eq:fh0p} \\
    \MoveEqLeft f^{+}_{\ell}(p^0_{\lm1},p_{\lm1}^+,q_{\ell}^-,w_\ell,\Lambda_{k\ell}^+)
    := \frac{1}{1-\alpha_{k\ell}^+} \nonumber \\
    & \times \left[
            h^{+}_{\ell}(p^0_{\lm1},p_{\lm1}^+,q_{\ell}^-,w_\ell,\theta_{k\ell}^+)
            - q^0_\ell - \alpha_{k\ell}^+ Q_\ell^- \right], \label{eq:fhp} \\
    \MoveEqLeft f^{-}_{L}(p^0_{\Lm1},p_{\Lm1}^+,w_L,\Lambda_{kL}^-)
    := \frac{1}{1-\alpha_{k\ell}^-}\nonumber \\
    &\times \left[
            h^{-}_{L}(p^0_{\Lm1},p_{\Lm1}^+,w_L,\theta_{kL}^-) - p^0_{\Lm1}
            - \alpha_{k,\Lm1}^- p_{\Lm1}^+ \right], \label{eq:fhLn}    \\
    \MoveEqLeft f^{-}_{\ell}(p^0_{\lm1},p_{\lm1}^+,q_{\ell}^-,w_\ell,\Lambda_{k\ell}^-)
    := \frac{1}{1-\alpha_{k,\lm1}^-} \nonumber \\
     &\times \left[
            h^{-}_{\ell}(p^0_{\lm1},p_{\lm1}^+,q_{\ell}^-,w_\ell,\theta_{k\ell}^-)
            - p^0_{\lm1}
            - \alpha_{k,\lm1}^- p_{\lm1}^+ \right]. \label{eq:fhn}
\end{align}
\end{subequations}
With these definitions, let $\fbf^{\pm}_\ell(\cdot)$ and $\hbf^{\pm}_\ell(\cdot)$
be the componentwise extensions of
$f^{\pm}_\ell(\cdot)$ and $h^{\pm}_\ell(\cdot)$.
It is then shown in \cite{fletcher2017inference} that the vectors
in \eqref{eq:pqdef} satisfy the recursions in the ``Forward" and ``Reverse" passes
of the transformed ML recursion in Algorithm~\ref{algo:trans}.

This is diagrammatically represented in the bottom panel of Fig.~\ref{fig:transformed}.
We see that, in the forward pass, the vectors are generated by an alternating sequence
of componentwise mappings where
\[
    \qbf^+_{k\ell} = \fbf^+_\ell(\pbf^+_{k,\lm1},\qbf^-_{k\ell},\cdots),
\]
followed by multiplication by $\Vbf_\ell$,
\[
    \pbf^+_{k\ell} = \Vbf_\ell \qbf^+_{k\ell}.
\]
Similarly, in the reverse pass, we have a componentwise mapping,
\[
    \pbf^-_{k\ell} = \fbf^-_{\lp1}(\pbf^+_{k\ell},\qbf^-_{k,\lp1},\cdots),
\]
followed by multiplication by $\Vbf_\ell\tran$,
\[
    \qbf^-_{k\ell} = \Vbf_\ell\tran \pbf^-_{k\ell}.
\]
Thus, similar to the MLP, we have written the forward and reverse passes of the
multi-layer updates as alternating sequence of componentwise (possibly nonlinear) functions
followed by multiplications by orthogonal matrices.


\subsection{SE Analysis}

Now that the variables and the ML-VAMP algorithm estiamtes are written in
the form of Algorithm~\eqref{algo:trans}, the
analysis of \cite{fletcher2017inference} to derive a simple state evolution.
Let
\begin{subequations} \label{eq:wdefvar}
\begin{align}
    W_0 &:= Z^0_0, \quad
    W_{\ell} := \Xi_\ell, \quad \ell =2,4,\ldots,L \\
    W_{\ell} &= (\bar{S}_{\ell},\bar{B}_\ell,\bar{\Xi}_\ell),  \quad \ell =1,3,\ldots,\Lm1,
\end{align}
\end{subequations}
where  $Z^0_0$, $\Xi_\ell$ and $(\bar{S}_{\ell},\bar{B}_\ell,\bar{\Xi}_\ell)$
are the random variable limits in \eqref{eq:varinitnl} and \eqref{eq:varinitlin}.
With these definitions, we can recursively define the random variables $Q_{k\ell}^{\pm}$
and $P_{k\ell}^{\pm}$ from the steps in Algorithm~\ref{algo:gen_se}.
This recursive definition of random variables is called the \emph{state evolution}.
We see that the SE updates in Algorithm~\ref{algo:gen_se} are in a one-to-one
correspondence with the steps in Transformed ML-VAMP algorithm, Algorithm~\ref{algo:trans}.
The key difference is that the SE updates involves \emph{scalar} random variables, as opposed 
to vectors.  The random variables are all either Gaussian random variables or the output of 
nonlinear function of the Gaussian random variables.  
In addition, the parameters of the Gaussians such as $\Kbf^+_{k\ell}$ and $\tau^-_{k\ell}$
are fully deterministic since they are computed via expectations.  

We now make further assumption:

\begin{assumption} \label{as:alpha}
Let $\alphabar_{k\ell}^{\pm}$ be generated by the SE recursions in Algorithm~\ref{algo:gen_se}.
Then  $\alphabar^{\pm}_{k\ell} \in (0,1)$ from the for all $k$ and $\ell$.
\end{assumption}




We can now state the main result.  The result includes Theorem~\ref{thm:mapse} as a special case.

\begin{theorem} \label{thm:genConv}  Let $\wbf_\ell, \pbf^{\pm}_{k\ell}$,
$\qbf^{\pm}_{k\ell}$, $\pbf^0_\ell$, $\qbf^0_\ell$
be defined as above.  Consider the sequence of random variables defined
by the SE updates in Algorithm~\ref{algo:gen_se} under the above assumptions.
Then,
\begin{enumerate}[(a)]
\item For any fixed $k$ and $\ell=1,\ldots,\Lm1$,
the parameter list $\Lambda_{k\ell}^+$ converges as
\beq \label{eq:Lamplim}
    \lim_{N \arr \infty} \Lambda_{k\ell}^+ = \Lambdabar_{k\ell}^+
\eeq
almost surely.
Also, the components of
$\wbf_\ell$, $\pbf^0_{\lm1}$, $\qbf^0_{\ell}$, $\pbf_{0,\lm1}^+,\ldots,\pbf_{k,\lm1}^+$ and $\qbf_{0\ell}^\pm,\ldots,\qbf_{k\ell}^\pm$
almost surely empirically converge jointly with limits,
\begin{align}
   \MoveEqLeft \lim_{N \arr \infty} \left\{
        (p^0_{\lm1,n},p^+_{i,\lm1,n},q^0_{\ell,n},q^-_{j\ell,n},q^+_{j\ell,n}) \right\} \nonumber \\
        &=
        (P^0_{\lm1},P^+_{i,\lm1},Q^0_{\ell},Q^-_{j\ell}, Q^+_{j\ell}), \label{eq:PQplim}
\end{align}
for all $i,j=0,\ldots,k$, where the variables
$P^0_{\lm1}$, $P_{i,\lm1}^+$ and $Q_{j\ell}^-$
are zero-mean jointly Gaussian random variables independent of $W_\ell$ with
\begin{align} \label{eq:PQpcorr}
\begin{split}
    &\Cov(P^0_{\lm1},P_{i,\lm1}^+) = \Kbf_{i,\lm1}^+, \quad \Exp(Q_{j\ell}^-)^2 = \tau_{j\ell}^-, \nonumber \\
    &\Exp(P_{i,\lm1}^+Q_{j\ell}^-)  = 0,  \quad \Exp(P^0_{\lm1}Q_{j\ell}^-)  = 0,
\end{split}
\end{align}
The identical result holds for $\ell=0$ with the variables $\pbf_{i,\lm1}^+$ and $P_{i,\lm1}^+$ removed.

\item For any fixed $k > 0$ and $\ell=1,\ldots,\Lm1$,
the parameter lists $\Lambda_{k\ell}^-$ converge as
\beq \label{eq:Lamnlim}
    \lim_{N \arr \infty} \Lambda_{k\ell}^- = \Lambdabar_{k\ell}^-
\eeq
almost surely.
Also, the components of
$\wbf_\ell$, $\pbf^0_{\lm1}$, $\pbf_{0,\lm1}^+,\ldots,\pbf_{\km1,\lm1}^+$, $\pbf_{0,\lm1}^+,\ldots,\pbf_{\km1,\lm1}^+$, and $\qbf_{0\ell}^-,\ldots,\qbf_{k\ell}^-$
almost surely empirically converge jointly with limits,
\begin{align}
    \MoveEqLeft \lim_{N \arr \infty} \left\{
        (p^0_{\lm1,n},p^+_{i,\lm1,n},q^-_{j\ell,n},q^+_{j\ell,n}) \right\} \nonumber \\
        &= (P^0_{\lm1},P^+_{i,\lm1},Q^-_{j\ell}, Q^+_{j\ell}), \label{eq:PQnlim}
\end{align}
for all $i=0,\ldots,\km1$ and $j=0,\ldots,k$, where the variables
$P^0_{\lm1}$, $P_{i,\lm1}^+$ and $Q_{j\ell}^-$
are zero-mean jointly Gaussian random variables independent of $W_\ell$ with
\begin{align} \label{eq:PQncorr}
\begin{split}
    & \Cov(P^0_{\lm1},P_{i,\lm1}^+) = \Kbf_{i,\lm1}^+,\quad
    \quad \Exp(Q_{j\ell}^-)^2 = \tau_{j\ell}^-, \\
    & \Exp(P_{i,\lm1}^+Q_{j\ell}^-)  = 0,
    \quad \Exp(P^0_{\lm1}Q_{j\ell}^-)  = 0,
\end{split}
\end{align}
The identical result holds for $\ell=L$ with all the variables $\qbf_{j\ell}^-$ and $Q_{j\ell}^-$ removed.
Also, for $k=0$, we remove the variables with $\pbf_{\km1,\ell}^+$ and $P_{\km1,\ell}^+$.
\end{enumerate}
\end{theorem}
\begin{proof}
This is proven almost identically to the result in \cite{fletcher2017inference}.
\end{proof}



\section{Numerical Experiments Details} \label{sec:simdetails}

\paragraph*{Synthetic random network}  The simulation is identical to \cite{fletcher2017inference},
except that we have run MAP ML-VAMP intead of MMSE ML-VAMP.  The details of the simulation are as follows:
As described in Section~\ref{sec:sim},
the network input is a $N_0=20$ dimensional Gaussian unit noise vector $\zbf_0$.
and has three hidden layers with 100 and 500 units and a variable number $N_y$ of
output units.  For the weight matrices and bias vectors
in all but the final layer,
we took $\Wbf_\ell$ and $\bbf_\ell$ to be random i.i.d.\ Gaussians.  The mean of the bias vector was selected
so that only a fixed fraction, $\rho=0.4$, of the linear outputs would be positive.  The activation
functions were rectified linear units (ReLUs), $\phi_\ell(z)=\max\{0,x\}$.  Hence, after activation,
there would be only a fraction $\rho=0.4$ of the units would be non-zero.  In the final layer,
we constructed the matrix similar to \citep{RanSchFle:14-ISIT} where $\Abf=\Ubf\Diag(\sbf)\Vbf\tran$,
with $\Ubf$ and $\Vbf$ be random orthogonal matrices and $\sbf$ be logarithmically spaced valued
to obtain a desired condition number of $\kappa=10$.  It is known from \citep{RanSchFle:14-ISIT}
that matrices with high condition numbers are precisely the matrices in which AMP algorithms fail.
For the linear measurements,
$\ybf = \Abf\zbf_5+\wbf$, the noise level $10\log_{10}( \Exp\|\wbf\|^2/\|\Abf\zbf_5\|^2)$ is set at 30 dB.
In Fig.~\ref{fig:randmlp_sim}, we have plotted the normalized MSE (in dB) which we define as
\[
    \mathrm{NMSE} := 10\log_{10}\left[ \frac{\|\zbf^0_0-\hat{\zbf}^{\pm}_{k0}\|^2}{\|\zbf^0_0\|^2} \right].
\]
Since each iteration of ML-VAMP involves a forward and reverse pass, we say that each iteration
consists of two ``half-iterations", using the same terminology as turbo codes.  The left panel
of Fig.~\ref{fig:randmlp_sim} plots the NMSE vs. half iterations.

\paragraph*{MNIST inpainting}  The well-known MNIST dataset consists of handwritten images
of size $28 \x 28 = 784$ pixels. We followed the procedure in \citep{kingma2013auto} for training
a generative model from 50,000 digits.
Each image $\xbf$ is modeled as the output of a neural network
input dimension of 20 variables followed by
a single hidden layer with 400 units and an output layer of 784 units,
corresponding to the dimension of the digits.
ReLUs were used for activation functions and a sigmoid was placed at the output
to bound the final pixel values between 0 and 1.
The inputs $\zbf^0_0$ were the modeled as zero mean Gaussians with unit variance.
The data was trained using the Adam optimizer
with the default parameters in TensorFlow
\footnote{Code for the training was based on
\url{https://github.com/y0ast/VAE-TensorFlow} by Joost van Amersfoort.}
The training optimization was run
with 20,000 steps with a batch size of 100 corresponding to 40 epochs.

The ML-VAMP algorithm was compared against MAP estimation.
As studied in \cite{yeh2016semantic,bora2017compressed}, MAP 
estimation can be performed via numerical minimization of the likelihood.
In this study, 
We used TensorFlow for the minimization.  We found the fastest
convergence with the Adam optimizer at a step-size of 0.01.  This required
only 500 iterations to be within 1\% of the final loss function.
For MAP ML-VAMP, the sigmoid
function does not have an analytic denoiser, so it was approximated with a probit output.
We found that the basic MAP ML-VAMP algorithm could be unstable.  Hence, damping 
as described in \citep{RanSchFle:14-ISIT} and \cite{rangan2017vamp} was used.
With damping, we needed to run the ML-VAMP algorithm for up to 500 iterations, which 
is comparable to the Adam optimizer.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> MLVAMP MAP/macros_parthe.tex <==
\newcommand{\pp}[1]{\textcolor{red}{#1}}

\newcommand{\mc}{\mathcal}
\newcommand{\ie}{\rm i.e.}
\newcommand{\T}{^\top}
\newcommand{\wb}[1]{\widebar{#1}}
